Testing software for non-discrimination: an updated and extended audit in the Italian car insurance domain

Context. As software systems become more integrated into society's infrastructure, the responsibility of software professionals to ensure compliance with various non-functional requirements increases. These requirements include security, safety, privacy, and, increasingly, non-discrimination. Motivation. Fairness in pricing algorithms grants equitable access to basic services without discriminating on the basis of protected attributes. Method. We replicate a previous empirical study that used black box testing to audit pricing algorithms used by Italian car insurance companies, accessible through a popular online system. With respect to the previous study, we enlarged the number of tests and the number of demographic variables under analysis. Results. Our work confirms and extends previous findings, highlighting the problematic permanence of discrimination across time: demographic variables significantly impact pricing to this day, with birthplace remaining the main discriminatory factor against individuals not born in Italian cities. We also found that driver profiles can determine the number of quotes available to the user, denying equal opportunities to all. Conclusion. The study underscores the importance of testing for non-discrimination in software systems that affect people's everyday lives. Performing algorithmic audits over time makes it possible to evaluate the evolution of such algorithms. It also demonstrates the role that empirical software engineering can play in making software systems more accountable.

==> tables/tab_average_comparison.tex <==
\begin{table}[!h]
\caption{Comparison of the results of the average rates analysis. The impact of features with \S will be deepened in Section \mrcomment{TODO: Inserire sezione in cui si discute}}
\label{tab_average-comparison}
\begin{tabular}{|l|p{6cm}|p{6cm}|}
\hline
\textbf{Features} & \textbf{Original study} & \textbf{New study} \\ \hline
Birthplace\S & Impact of the price were proven for non-Italian profiles. & Impact of the price were proven for different non-Italian profiles. \\ \hline
Marital status\S & Was not tested. & Seems to play a negligible role. \\ \hline
Profession\S & Was not tested. & Seems to play a negligible role. \\ \hline
Education\S & Was not tested. & Seems to play a negligible role. \\ \hline
Gender & Seems to play a negligible role. & Seems to play a negligible role. \\ \hline
Age & Seems to play a negligible role. & Seems to play a negligible role. \\ \hline
Km driven & Seems to play a negligible role. & Seems to play a negligible role. \\ \hline
Class & Impact on the price was confirmed but justified. & Impact on the price was confirmed but justified. \\ \hline
Car & Impact on the price was confirmed but justified. & Impact on the price was confirmed but justified. \\ \hline
City & The impact on the price was confirmed. & The impact on the price was negligible. \\ \hline
\end{tabular}
\end{table}
